The Covariant Phase Space of Gravity with Boundaries

This thesis investigates how the metric and tetrad formulations of three gravitational field theories in manifolds with timelike boundaries within the covariant phase space program. With the recently developed relative bicomplex framework, we explore the space of solutions and presymplectic structures associated with each action principle and analyse their equivalence. In this way, the relative bicomplex surpasses traditional covariant phase space methods, which are only suited for boundary-free field theories.

==> preface.tex <==
\chapter*{Preface}
 

